Scalable Tail Latency Estimation for Data Center Networks

In this paper, we consider how to provide fast estimates of flow-level tail latency performance for very large scale data center networks. Network tail latency is often a crucial metric for cloud application performance that can be affected by a wide variety of factors, including network load, inter-rack traffic skew, traffic burstiness, flow size distributions, oversubscription, and topology asymmetry. Network simulators such as ns-3 and OMNeT++ can provide accurate answers, but are very hard to parallelize, taking hours or days to answer what if questions for a single configuration at even moderate scale. Recent work with MimicNet has shown how to use machine learning to improve simulation performance, but at a cost of including a long training step per configuration, and with assumptions about workload and topology uniformity that typically do not hold in practice. We address this gap by developing a set of techniques to provide fast performance estimates for large scale networks with general traffic matrices and topologies. A key step is to decompose the problem into a large number of parallel independent single-link simulations; we carefully combine these link-level simulations to produce accurate estimates of end-to-end flow level performance distributions for the entire network. Like MimicNet, we exploit symmetry where possible to gain additional speedups, but without relying on machine learning, so there is no training delay. On large-scale networks where ns-3 takes 11 to 27 hours to simulate five seconds of network behavior, our techniques run in one to two minutes with 99th percentile accuracy within 9% for flow completion times.

==> background.tex <==
\section{Background and Motivation}

\kz{
    full-fidelity simulation slow because dependencies between events have to
    be respected, reducing chances for parallelization.
    also it's slow because application, transport, network, and link layers are
    modeled. even if you don't need them you still pay for them out of the box.
    full-fidelity simulation cannot be effectively parallelized (MimicNet).
    flow-level approximations: most assume flows reach steady-state
    immediately, then solve a bandwidth sharing problem. this becomes less
    accurate with higher link speeds (MimicNet eval used 100Mbps, and it still
    wasn't accurate).
    don't know of any flow-level simulators that model queues; don't want to
    claim too much here.
    maybe more comments on MimicNet.
}

==> discussion.tex <==
\section{Discussion}

\kz{
    From Mohammad: maybe slightly-longer-than-usual discussion of what you
    could use this for.
}

==> relwork.tex <==
\section{Related Work}
